Soft Adaptive Feet for Legged Robots: An Open-Source Model for Locomotion Simulation

In recent years, artificial feet based on soft robotics and under-actuation principles emerged to improve mobility on challenging terrains. This paper presents the application of the MuJoCo physics engine to realize a digital twin of an adaptive soft foot developed for use with legged robots. We release the MuJoCo soft foot digital twin as open source to allow users and researchers to explore new approaches to locomotion. The work includes the system modeling techniques along with the kinematic and dynamic attributes involved. Validation is conducted through a rigorous comparison with bench tests on a physical prototype, replicating these experiments in simulation. Results are evaluated based on sole deformation and contact forces during foot-obstacle interaction. The foot model is subsequently integrated into simulations of the humanoid robot COMAN+, replacing its original flat feet. Results show an improvement in the robot's ability to negotiate small obstacles without altering its control strategy. Ultimately, this study offers a comprehensive modeling approach for adaptive soft feet, supported by qualitative comparisons of bipedal locomotion with state of the art robotic feet.

==> Introduction.tex <==
\section{INTRODUCTION}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%% NEW INTRO INCLUDING OPEN-SOURCE TOPIC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Replicating human locomotion and stability on uneven terrains has been a longstanding challenge in robotics. Flat-footed (e.g. ATLAS, Digit, HRP-4 \cite{Caron2019}, H1, Nao, WALK-MAN \cite{Negrello}), and passive ball-shaped (e.g. ANYmal \cite{Hutter2016}, HyQ \cite{Boaventura2013}, MIT Cheetah \cite{Bledt2018}, Spot) robots often struggle to traverse irregular terrains, limiting their applications in unstructured environments. 

\par Humanoid feet exhibit various structural designs. However, most commonly, they feature either a single rigid segment or two segments connected by a revolute joint. Nonetheless, more complex designs have been developed to enhance their adaptability to diverse terrains, making them suitable for tasks requiring stability and agility.
% Soft adaptive feet, inspired by principles of soft robotics, have been developed because of their exceeding capability to adapt to diverse terrains, making them suitable for tasks requiring stability and agility.
%
Examples include foot soles embodying compliant visco-elastic materials \cite{Owaki2012, dema2017sole, Nikos2015, Isozumi2002}, or airbag units to absorb small ground irregularities \cite{Najmuddin2012, Zang2017}. Other feet use more articulated structures consisting of multiple segments connected by joints and compliant elements \cite{Seo2009ModelingAA, Takanishi2010, Davis2010TheDO, Inaba2016}.
%
Our team adopted a different approach, instead, for developing an adaptive robotic passive foot, i.e. the SoftFoot: ground adaptability is tackled directly at a mechanical level, through the design of an elastic and deformable sole replicating that of the human counterpart \cite{Piazza2024}. When tested on the humanoid robot HRP-4 stepping on small obstacles, it led to notable stability and obstacle negotiation improvements \cite{Catalano2021hrp4}.
% An increased stability was reported also with the prototype specifically devised for quadrupeds, i.e. the SoftFoot-Q \cite{Catalano2021quad}.

% \par A similar soft foot design may greatly benefit the prosthetic community too. Despite the recent technological developments in the field (some research prototypes can be found in \cite{Weerakkody2017}), indeed, lower-limb prosthetic users still find challenging walking on uneven terrains, with an associated risk of falls \cite{kim2022} and a decreased quality of life \cite{Hagberg2001}. 

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{img/SF_robotico_model.png} 
    \caption{Robotic SoftFoot prototype. On the left a picture of the physical foot, on the right a rendering of the SoftFoot MuJoCo model.\vspace{-2mm}}
    \label{fig:model}
\end{figure}

% \par In addition, the development of adaptive designs has enabled new control strategies exploiting data related to foot deformation to dynamically adjust gait, contact forces, and stability in real time. Examples, where the sole deformation acts as feedback for innovative walking algorithms, can be found in \cite{dema2017control, Pajon2017, Owaki2012}.

\par 
% Albeit the advantages provided by soft technologies in terms of enhanced adaptability, their complex mechanical structure entails an increased mathematical complexity. Analytical models struggle to account for the inherent dynamic interactions, uncertainties, and nonlinearities present in complex robotic systems. Thus, they often rely on simplifications and assumptions to be mathematically tractable.
While soft technologies offer enhanced adaptability, their complex mechanical structures introduce signifFicant mathematical challenges. Analytical models often struggle to accurately represent the dynamic interactions, uncertainties, and nonlinearities inherent in such systems, necessitating simplifications and assumptions for mathematical tractability.
For instance, ball-shaped feet are often simplified to a single contact point with the ground \cite{Kim2016}; pressure changes in airbags are assumed to be isothermal \cite{Zang2017}; the SoftFoot model to evaluate the contact forces distribution on its sole works under specific assumptions \cite{Mura2020}. 
% The dynamics associated with the use of soft technologies generally prove to be nontrivial to describe \cite{Armanini2023}.

Physics engines offer a valuable alternative to analytical models with several advantages. They provide, indeed, a dynamic and realistic virtual environment in which sophisticated robotic systems can be replicated and tested. They ease the design process and facilitate real-time testing and optimization of both the mechanical design and control architecture. Notable examples of applications include very complex and contact-rich tasks, like a robotic hand solving a Rubik's cube \cite{OpenAI2019} and manipulation tasks for industrial robots \cite{Yoon2023}, or testing control architecture on a humanoid robot \cite{Gentiane2022}.
% Applications extend to soft bodies (e.g. \cite{Hu2019}), and to human biomechanical control too (e.g. \cite{Caggiano2022}). 
Several physics engines are available, including Bullet, ODE, PhysX, MuJoCo, and Havok. Studies have evaluated these for specific and general robotics applications \cite{Roennau2013, Erez2015, Ivaldi2015, Liu2021}, but no single engine stands out as the best. Simulator selection should, therefore, depend on the specific task and required features.
% Several physics engines are currently available, such as Bullet, ODE, PhysX, MuJoCo, and Havok. Some studies have tried to identify the most appropriate for both specific and more general applications in robotics \cite{ Roennau2013, Erez2015, Ivaldi2015,Liu2021}. Apparently, there is not a singular winner, so the simulator selection should be based on the intended simulation task and the desired features.
MuJoCo proved to work fast and accurately with constrained systems \cite{Erez2015}. It offers support for rigid-body dynamics, friction, and contact modeling, focusing on classical robotics applications as well as on the simulation of humanoid robots \cite{Ivaldi2015}. 
% It is also well-suited for control optimization, and enables real-time integration within control loops \cite{Todorov2014}.
% Last but not least, it allows for modeling non-flat rigid terrains and with various textures, enhancing its versatility in simulating different environments.

%%%%%% DIGITAL TWIN %%%%%%%%
The concept of digital twins has gained prominence when addressing the complexity of modeling soft robotics systems \cite{Tammi2019, Leng2017, Sahin2021, Li2021}. Digital twins are virtual representations of physical objects or systems that enable real-time monitoring, analysis, and optimization. By creating a digital twin of a soft robotic foot, it is possible to simulate its behavior in various scenarios, predict performance outcomes, and iteratively refine its design and control strategies. 
% This approach not only enhances understanding but also expedites the development process by reducing the need for physical prototypes and extensive testing.

%Why MuJoCo? Here and not in methods!
%%%%%%%%%%%%%%%%%%%%%%% What about our work here? What, why, how, chapter definition. %%%%%%%%%%%%%%%%%%%%
In this work, we present a comprehensive model of the SoftFoot developed within the MuJoCo physics engine, given its capability to handle contacts and constrained systems.  
The model serves for analyzing the interaction of the SoftFoot with uneven terrains and obstacles and for design development and it will be released as open-source within the Natural Machine Motion Initiative \cite{dellasantina2017}.
% in addition to the open hardware drawing of the SoftFoot already released on the same open platform.
% By using a simulator, we avoid making strong assumptions and simplifications, as in \cite{Mura2020}, to better approximate the foot performance in the real world. (magari spostare nelle discussioni?)

The paper presents the model description within the simulator (Section II), as well as its validation (Section III) conducted by replicating in simulation a bench-testing previously performed with the same foot prototype \cite{Mura2020}. Foot sole deformation and contact forces with the obstacles are used as the metric to assess model accuracy and performance (Section IV).
% Additionally, we performed a qualitative analysis of a more dynamic task, such as bipedal locomotion, to show the effectiveness of SoftFoot compared to rigid feet, as in \cite{Catalano2021hrp4}. 
Additionally, we reproduce in the simulator a locomotion task of a humanoid robot walking with SoftFoot, such as that described in \cite{Catalano2021hrp4}, to qualitatively analyze the effectiveness of the adaptive foot in negotiating obstacles.




